O-Dang! The Ontology of Dangerous Speech Messages

Inside the NLP community there is a considerable amount of language resources created, annotated and released every day with the aim of studying specific linguistic phenomena. Despite a variety of attempts in order to organize such resources has been carried on, a lack of systematic methods and of possible interoperability between resources are still present. Furthermore, when storing linguistic information, still nowadays, the most common practice is the concept of "gold standard", which is in contrast with recent trends in NLP that aim at stressing the importance of different subjectivities and points of view when training machine learning and deep learning methods. In this paper we present O-Dang!: The Ontology of Dangerous Speech Messages, a systematic and interoperable Knowledge Graph (KG) for the collection of linguistic annotated data. O-Dang! is designed to gather and organize Italian datasets into a structured KG, according to the principles shared within the Linguistic Linked Open Data community. The ontology has also been designed to account for a perspectivist approach, since it provides a model for encoding both gold standard and single-annotator labels in the KG. The paper is structured as follows. In Section 1 the motivations of our work are outlined. Section 2 describes the O-Dang! Ontology, that provides a common semantic model for the integration of datasets in the KG. The Ontology Population stage with information about corpora, users, and annotations is presented in Section 3. Finally, in Section 4 an analysis of offensiveness across corpora is provided as a first case study for the resource.

==> appunti_vari.tex <==
{\color{blue}
\section{Introduction/Motivation}
MOTIVZIONE (1): Within the computational social science community, there is a growing awareness for the benefits of a larger body of diverse datasets covering multiple languages and platforms, rather than assuming that datasets on highly resourced languages like English (or easily shared platforms like Twitter) are representative of human language as a whole (Bender, 2011; Tufekci, 2014, inter alia).\\

MOTIVAZIONE (2): providing a discussion forum about the usage of Linguistic Linked Data principles in the Sentiment Analysis field, to explore relevant principles, methodologies, resources, tools and applications, and understand the primary approaches, their advantages, limitations, and the available resources and case studies.\\
}

\section{Linguistic Linked Open Data}
The Linguistic Linked Open Data (LLOD) Cloud\footnote{\url{https://linguistic-lod.org/}} \cite{chiarcos2011towards,mccrae2016open,declerck2020recent} promotes interoperability and reusability of resources for NLP. Rather than being just a hub of corpora and lexicons, LLOD Cloud identifies guidelines and standards to model linguistic data set according to the Semantic Web principles \cite{berners2001semantic}. Hence, corpora must be developed as KGs to be stored in the LLOD Cloud. Moreover, the Ontolex-Lemon ontology \cite{buitelaar2011ontology,mccrae2017ontolex} was provided as a standard for the encoding of lexical resources. This semantic model reifies the interplay between a lexical entries and their meaning. For instance, the word ``wedding'' in the sentence ``The wedding of Prince Charles and Lady Diana Spencer took place on Wednesday, 29 July 1981'' from Wikipedia is stored as a \textsc{ontolex:LexicalEntry} with a \textsc{ontoloex:LexicalSense} that may be its meaning on WordNet or other vocabularies. The lexical sense is in turn linked with a \textsc{ontolex:Reference}, namely the source of knowledge where the lexical entry occurred, and to a more abstract \textsc{ontolex:LexicalConcept} ``Wedding'', that includes several forms of the same meaning, such as ``marriage'' and ``matrimony''. That kind of modeling is highly explainable since it draws an explicit semantic relation between lexical items and their means. Moreover, it potentially eases the mapping between several corpora. 

Many resources have been released according to LLOD principles in last years: \newcite{mccrae2014publishing} developed a RDF version of WordNet, \newcite{chiarcos2017conll} provided the CoNLL-RDF infrastracture, \newcite{passarotti2019lila} released LiLa, a Knowledge base of linguistic resources for Latin. Notwithstanding, models aimed at mapping corpora annotated for abusive language are still missing, despite the large number of existing data set and the variety of annotation schemes \cite{poletto2021resources}. 

Our work tries to fill this gap by releasing a semantic model for representing stereotypes and correlated phenomena (see Section \ref{sec:ontology}). The model, mapped with Ontolex-Lemon \cite{mccrae2014publishing}, was designed to easily align several types of data, sources of knowledge and annotation schemes in a unique formal representation. Moreover, it was conceived to release annotations in a non-aggregated form, promoting the study of subjectivity relevant to this phenomena and following a perspectivist approach \hl{(inserire reference)}.

\section{A Semantic Model of Stereotype} \label{sec:ontology}
\begin{figure*}
  \includegraphics[width=0.95\textwidth]{overview_stereotipi_tratteggio.png}
  \caption{Overview stereotipi}
  \label{img:overview_stereotipi}
\end{figure*}

\begin{figure*}
  \includegraphics[width=0.95\textwidth]{nuovo_esempio_stereotipo.png}
  \caption{Esempio stereotipo}
  \label{img:esempio_stereotipo}
\end{figure*}
The Semantic Model for encoding stereotypes and correlated phenomena must fulfill three needs:

\begin{enumerate}
    \item organizing many types of contents (eg: texts, images, videos) gathered from different sources;
    \item providing information about agents involved in the diffusion and evaluation of a stereotypes;
    \item proposing a common format for aligning several annotation schemes about stereotypes and other correlated phenomena.
\end{enumerate}

The first two are described in this section, while the third is presented in Section \ref{sec:KG} together with the annotation pipeline that led to the creation of the Ster-KG
    
\smallskip
\paragraph{Organizing contents.} FRBR\footnote{\url{http://purl.org/spar/frbr}} \citelanguageresource{tillett2005frbr}, FaBiO\footnote{\url{http://purl.org/spar/fabio/2018-05-02}} \citelanguageresource{peroni2012fabio}, DOLCE\footnote{\url{http://ontologydesignpatterns.org/wiki/Ontology:DOLCE+DnS_Ultralite}} \citelanguageresource{gangemi2002sweetening} ontologies, and Dublin Core vocabulary\footnote{\url{http://purl.org/dc/elements/1.1/}} \citelanguageresource{weibel1997dublin} were reused to model the first information. As it can be observed in the upper part of Figure \ref{img:overview_stereotipi}, the more abstract representation of the relation between expressions and stereotypes relies on DOLCE, an upper ontology which constitutes an authoritative source of knowledge for our work. Each expression (eg: a text, an image) is a \textsc{dul:InformationObject} that expresses a \textsc{dul:Concept}, in our case a stereotype. FRBR further specializes this interplay representing the distinction between a \textsc{frbr:Expression} and a \textsc{frbr:Manifestation}. The former is equivalent to an information object while the latter informs about its specific embodiment. Hence, a \textit{tweet} is the manifestation of a text, and an image is an expression that could have a manifestation on Instagram. Such a distinction may be useful to represent data gathered from different sources or to analyze how the same expression is perceived in different communication environment. A taxonomy of expressions is provided by Dublin Core, whereas FaBiO adds to the ontology a list of manifestations. Our KG includes a data set of the type \textsc{dc:Text} that is embodied as a Tweet \textsc{fabio:WebContent} and expresses a \textsc{ster:Stereotype}.

\smallskip
\paragraph{Providing information about agents.} Condition such as being an annotator, the addresser of a message, or the target of a stereotype are all anti-rigid properties \cite{guarino2004overview}, and they have being encoded as roles associated to agents. For instance, an agent may play the role of addresser, and this role is associated with a particular stereotype. The same agent may hold the role of target and associated to another stereotype. We adopted the \textbf{dul:hasRole} property from DOLCE, and integrated the PROV-O ontology\footnote{\url{https://www.w3.org/TR/prov-o/}} \cite{lebo2013prov} in our model to express the provenance of information about stereotypes. From this resource we reused the taxonomy of agents - \textsc{prov:Person}, \textsc{prov:Group}, \textsc{prov:Organization}, \textsc{prov:SoftwareAgent} - and the property \textbf{prov:wasAttributedTo} that links roles and stereotypes. $4$ roles were defined in the ontology. 

\textsc{ster:Addresser} and \textsc{ster:Addressee} are derived from Jakobson's theory of communication \cite{jakobson1987language} and refer to the sender of a message, and their eventual recipient. \textsc{ster:Target} is the group of people towards which a stereotype is directed. Examples of addressees in our KG are users mentioned at the beginning of the tweet, while the target is the agent of the annotated stereotype.

The role of \textsc{prov:Annotator} has two functions in the ontology (see the lower part of Figure \ref{img:overview_stereotipi}). It attributes the annotator and their demographic features to all their annotations and clustering. The excerpt of RDF triples below exemplifies how this information is stored in the KG. First, an entity of the type \textsc{ster:Annotation} is attributed to its annotator and linked to \textsc{ster:Dangerous}, a subclass of \textsc{ster:Stereotype}, through the property \textbf{ster:wasClusteredAs}. Then \textsc{ster:Dangerous} is attributed with the annotator who defined this class of the ontology. Finally, demographic information about the \textsc{prov:Person} who had the role of \textsc{ster:Annotator} for this annotation are provided.

{\small \begin{verbatim}
    
`i migranti sono pericolosi' a 
ster:Annotation;
prov:wasAttributedTo annotator_02;
ster:wasClusteredAs ster:Dangerous.
ster:Dangerous rdfs:SubClassOf 
ster:Stereotype;
prov:wasAttributetTo annotator_02.
annotator_02 a Annotator;
dul:isRoleOf prov:Person;
ster:gender ``female'';
ster:age 29;
ster:birthCountry ster:Italy.
\end{verbatim}}

\section{Corpus Creation and Description} \label{sec:KG}

The corpus creation stage was a two-step annotation process of a sample from The Hate Speech Detection Task \cite{sanguinetti2020haspeede} data set. We selected $1,000$ texts, half of which labelled as containing stereotype and Hate Speech, while the other only stereotype. 

The first part on the task was devoted to enrich the existing sample with a finer grained annotation of stereotype. $5$ annotators were asked to select one or more chunk from each Twitter post and label them with at least one minimum phrase of the form S-V-O or S-NP. Phrases had to include both the target group and the stereotype like in `Gli immigrati sono privilegiati'\footnote{Migrants are privileged}. 

Such annotation scheme emphasizes the annotators subjectivity, since it is not a rigid predetermined set of labels. However it does not allow for delivering a traditional gold standard corpus, that would be also incompatible with this approach. In order to overcome the issue, we asked annotators to group the minimum phrases they formulated first in $10$, then in $5$ clusters.

Figure \ref{img:esempio_stereotipo} depicts the internal structure of an annotated stereotypes as it is represented in the ontology. Each annotation is mapped with the Ontolex-Lemon model \cite{mccrae2017ontolex} and structured in three components. \textsc{ontolex:LexicalEntry} is the chunk of text selected by the annotator. In our example the sentence ``imputati stranieri vengono tutti a delinquere''\footnote{foreign accused all come to commit crimes} is part of a wider Twitter post. The \textsc{ster:Annotation} is a minimum phrase formulated by the annotator to indicate the stereotype expressed by the chunk: ``gli immigrati sono delinquenti''\footnote{Immigrants are criminal}. It is a subclass of \textsc{ontolex:LexicalSense} conveying the sense of \textsc{ontolex:LexicalEntry}. It works as a link between the chunk and the more comprehensive \textsc{ontolex:LexicalConcept} ``SonoPericolosi''\footnote{Dangerous}. The latter was not modeled prior to the annotation, but it is the outcome of a clustering provided by annotators to reduce the variety of minimum phrases expressing stereotypes. Hence, minimum phrases such as `gli immigrati sono stupratori'\footnote{Migrants are rapists}, `i rom spacciano'\footnote{Roma people sell drugs}, `i mussulmani sono una minaccia'\footnote{Muslims are a threat} were all clustered in the same stereotypical \textsc{ontolex:LexicalConcept} ``SonoPericolosi''\footnote{Dangerous}, splitting the stereotype from the target group.

The same mapping is represented in the following RDF triples, which also express the attribution relation between annotations and annotators through the property \textbf{prov:wasAttributedTo}, and the target of the stereotypes through the property \textbf{ster:hasTarget}.

{\small
\begin{verbatim}
    [ 
    a ontolex:LexicalEntry;
    ster:chunk ``imputati stranieri 
    vengono tutti a delinquere'';
    dul:isPartOf fabio:WebContent;
    prov:wasAttributedTo annotator_02
    ontolex:sense [
    a ster:Annotation,
    ontolex:LexicalSense;
    ster:frame ``gli immigrati sono
    delinquenti'';
    ontolex:isLexicalizedSenseOf [
    a ster:Dangerous;
    rdfs:subClassOf ster:Stereotype,
    ontolex:LexicalConcept.
    ster:hasTarget ster:minorities;
    prov:wasAttributedTo annotator_01;
    
            ]
        ]
    ]
\end{verbatim}
}
